Obtaining Structural Network Controllability with Higher-Order Local Dynamics

We consider a network of identical, first-order linear systems, and investigate how replacing a subset of the systems composing the network with higher-order ones, either taken to be generic or specifically designed, may affect its controllability. After establishing a correspondence between state controllability in networks of first-order systems with output controllability in networks of higher-order systems, we show that adding higher-order dynamics may require significantly fewer subsystem modifications to achieve structural controllability, when compared to first-order heterogeneous subsystems. Furthermore, we characterize the topology of networks (which we call X-networks) in which the introduction of heterogeneous local dynamics is not necessary for structural output controllability, as the latter can be attained by suitable higher-order subsystems with homogeneous internal dynamics.

==> img/tree/tree.tex <==
\begin{tikzpicture}
\begin{scope}
    

\node[draw,circle,thick,scale=0.7,inner sep=0.05cm] (1) at (0,0) {1};
\node[draw,circle,thick,scale=0.7,inner sep=0.05cm] (2) at (-0.7,-0.75) {2};
\node[draw,circle,fill=RoyalBlue!20,thick,scale=0.7,inner sep=0.05cm] (3) at (0.7,-0.75) {3};
\node[draw,circle,thick,scale=0.7,inner sep=0.05cm] (4) at (-1.3,-1.5) {4};
\node[draw,circle,fill=RoyalBlue!20,thick,scale=0.7,inner sep=0.05cm] (5) at (-0.3,-1.5) {5};
\node[draw,circle,fill=RoyalBlue!20,thick,scale=0.7,inner sep=0.05cm] (6) at (0.3,-1.5) {6};
\node[draw,circle,fill=RoyalBlue!20,thick,scale=0.7,inner sep=0.05cm] (7) at (1.3,-1.5) {7};
\node[draw,circle,thick,scale=0.7,inner sep=0.145cm]  at (-1.55,-2.5) {};
\node[draw,circle,fill=RoyalBlue!20,thick,scale=0.7,inner sep=0.145cm]  at (-1.05,-2.5) {};
\node[draw,circle,fill=RoyalBlue!20,thick,scale=0.7,inner sep=0.145cm]  at (0.5,-2.5) {};
\node[draw,circle,fill=RoyalBlue!20,thick,scale=0.7,inner sep=0.145cm]  at (1.05,-2.5) {};
\node[draw,circle,fill=RoyalBlue!20,thick,scale=0.7,inner sep=0.145cm]  at (1.55,-2.5) {};
\node  at (-0.25,-2.5) {\dots};
\node[draw,circle,thick,scale=0.7,inner sep=0.05cm] (u) at (-0.5,0.5) {$u$};
\draw[semithick,{|}-{|}] (-1.9, 0) -- (-1.9,-2.5);
\node[inner sep=0cm] at (-1.7,-1) {$h$};
\node[inner sep=0cm] at (2.5,-1.25) {\ };

% \draw [-stealth,
% line join=round,
% semithick,
% decorate, decoration={
%     zigzag,
%     segment length=4,
%     amplitude=.9,post=lineto,
%     post length=2pt
% }]  (-0.5,0.5) node[left] {$u$}-- (1);
\draw[-stealth,semithick,line join=round,
semithick,
decorate, decoration={
    zigzag,
    segment length=4,
    amplitude=.9,post=lineto,
    post length=2pt
}] (u) -- (1);
\draw[-stealth,semithick] (1) -- (2);
\draw[-stealth,semithick] (1) -- (3);
\draw[-stealth,semithick] (2) -- (4);
\draw[-stealth,semithick] (2) -- (5);
\draw[-stealth,semithick] (3) -- (6);
\draw[-stealth,semithick] (3) -- (7);
\draw[dashed,semithick] (4) -- (-1.5,-2.25);
\draw[dashed,semithick] (4) -- (-1.1,-2.25);
\draw[dashed,semithick] (5) -- (-0.5,-2.25);
\draw[dashed,semithick] (5) -- (-0.1,-2.25);
\draw[dashed,semithick] (6) -- (0.5,-2.25);
\draw[dashed,semithick] (6) -- (0.1,-2.25);
\draw[dashed,semithick] (7) -- (1.5,-2.25);
\draw[dashed,semithick] (7) -- (1.1,-2.25);


\node at (0,-3) {(a)};
\node at (0,1) {binary tree};
\end{scope}
\begin{scope}[xshift=125]
    
\node[draw=red,fill=BrickRed!10,minimum width=1.1cm,minimum height=0.5cm] at (0,0) {};
\node[draw,circle,fill=ForestGreen!20,thick,scale=0.7,inner sep=0.05cm] (1) at (-0.3,0) {1};
\node[draw,circle,fill=white,thick,scale=0.7,inner sep=0.05cm] (1b) at (0.3,0) {2};
\node[draw=red,fill=BrickRed!10,minimum width=1.1cm,minimum height=0.5cm] at (-0.9,-0.75) {};
\node[draw,circle,fill=ForestGreen!20,thick,scale=0.7,inner sep=0.05cm] (2) at (-1.2,-0.75) {3};
\node[draw,circle,fill=white,thick,scale=0.7,inner sep=0.05cm] (2b) at (-0.6,-0.75) {4};
\node[draw=red,fill=BrickRed!10,minimum width=1.1cm,minimum height=0.5cm] at (1,-0.75) {};
\node[draw,circle,fill=ForestGreen!20,thick,scale=0.7,inner sep=0.05cm] (3) at (0.7,-0.75) {5};
\node[draw,circle,fill=white,thick,scale=0.7,inner sep=0.05cm] (3b) at (1.3,-0.75) {6};
\node[draw=red,fill=BrickRed!10,minimum width=1.1cm,minimum height=0.5cm] at (-1.8,-1.5) {};
\node[draw,circle,fill=ForestGreen!20,thick,scale=0.7,inner sep=0.05cm] (4) at (-2.1,-1.5) {7};
\node[draw,circle,fill=white,thick,scale=0.7,inner sep=0.05cm] (4b) at (-1.5,-1.5) {8};
\node[draw=red,fill=BrickRed!10,minimum width=1.1cm,minimum height=0.5cm] at (-0.6,-1.5) {};
\node[draw,circle,fill=ForestGreen!20,thick,scale=0.7,inner sep=0.05cm] (5) at (-0.9,-1.5) {9};
\node[draw,circle,fill=white,thick,scale=0.575,inner sep=0.05cm] (5b) at (-0.3,-1.5) {10};
\node[draw=red,fill=BrickRed!10,minimum width=1.1cm,minimum height=0.5cm] at (0.6,-1.5) {};
\node[draw,circle,fill=ForestGreen!20,thick,scale=0.575,inner sep=0.05cm] (6) at (0.3,-1.5) {11};
\node[draw,circle,fill=white,thick,scale=0.575,inner sep=0.05cm] (6b) at (0.9,-1.5) {12};
\node[draw=red,fill=BrickRed!10,minimum width=1.1cm,minimum height=0.5cm] at (1.8,-1.5) {};
\node[draw,circle,fill=ForestGreen!20,thick,scale=0.575,inner sep=0.05cm] (7) at (1.5,-1.5) {13};
\node[draw,circle,fill=white,thick,scale=0.575,inner sep=0.05cm] (7b) at (2.1,-1.5) {14};
\node[draw,circle,fill=ForestGreen!20,thick,scale=0.7,inner sep=0.145cm]  at (-2.25,-2.5) {};
\node[draw,circle,fill=ForestGreen!20,thick,scale=0.7,inner sep=0.145cm]  at (-1.65,-2.5) {};
\node[draw,circle,fill=ForestGreen!20,thick,scale=0.7,inner sep=0.145cm]  at (1.05,-2.5) {};
\node[draw,circle,fill=ForestGreen!20,thick,scale=0.7,inner sep=0.145cm]  at (1.65,-2.5) {};
\node[draw,circle,fill=ForestGreen!20,thick,scale=0.7,inner sep=0.145cm]  at (2.25,-2.5) {};
\node  at (-0.25,-2.5) {\dots};
\node[draw,circle,thick,scale=0.7,inner sep=0.05cm] (u) at (-0.8,0.5) {$u$};


\draw[-stealth,semithick,line join=round,
semithick,
decorate, decoration={
    zigzag,
    segment length=4,
    amplitude=.9,post=lineto,
    post length=2pt
}] (u) -- (1);

\draw[-stealth,semithick] (1) to[bend left=20] (1b);
\draw[-stealth,semithick] (1b) to[bend left=20] (1);
\draw[-stealth,semithick] (2) to[bend left=20] (2b);
\draw[-stealth,semithick] (2b) to[bend left=20] (2);
\draw[-stealth,semithick] (3) to[bend left=20] (3b);
\draw[-stealth,semithick] (3b) to[bend left=20] (3);
\draw[-stealth,semithick] (4) to[bend left=20] (4b);
\draw[-stealth,semithick] (4b) to[bend left=20] (4);
\draw[-stealth,semithick] (5) to[bend left=20] (5b);
\draw[-stealth,semithick] (5b) to[bend left=20] (5);
\draw[-stealth,semithick] (6) to[bend left=20] (6b);
\draw[-stealth,semithick] (6b) to[bend left=20] (6);
\draw[-stealth,semithick] (7) to[bend left=20] (7b);
\draw[-stealth,semithick] (7b) to[bend left=20] (7);
\draw[-stealth,semithick] (1) -- (2);
\draw[-stealth,semithick] (1b) -- (3);
\draw[-stealth,semithick] (2) -- (4);
\draw[-stealth,semithick] (2b) -- (5);
\draw[-stealth,semithick] (3) -- (6);
\draw[-stealth,semithick] (3b) -- (7);
\draw[dashed,semithick] (4) -- (-2.2,-2.25);
\draw[dashed,semithick] (4b) -- (-1.6,-2.25);
\draw[dashed,semithick] (5) -- (-1,-2.25);
\draw[dashed,semithick] (5b) -- (-0.4,-2.25);
\draw[dashed,semithick] (6b) -- (1,-2.25);
\draw[dashed,semithick] (6) -- (0.4,-2.25);
\draw[dashed,semithick] (7b) -- (2.2,-2.25);
\draw[dashed,semithick] (7) -- (1.6,-2.25);


\node at (0,-3) {(b)};
\node at (0,1) {lifted binary tree};

\end{scope}
\end{tikzpicture}
